A Survey on Semantic Parsing

A significant amount of information in today's world is stored in structured and semi-structured knowledge bases. Efficient and simple methods to query them are essential and must not be restricted to only those who have expertise in formal query languages. The field of semantic parsing deals with converting natural language utterances to logical forms that can be easily executed on a knowledge base. In this survey, we examine the various components of a semantic parsing system and discuss prominent work ranging from the initial rule based methods to the current neural approaches to program synthesis. We also discuss methods that operate using varying levels of supervision and highlight the key challenges involved in the learning of such systems.

==> Semantic parsing survey/sections/early_attempts.tex <==
\subsection{Rule based systems}
Early semantic parsing systems were mainly rule-based, making them domain specific. These can be based on pattern matching such as \texttt{SAVVY} \cite{johnson1984natural} which although simple, is quite brittle due to the shallow nature of the pattern matching. 
% \citet{androutsopoulos1995natural} mentions an example where the query ``\texttt{TITLES OF EMPLOYEES IN LOS ANGELES}" to SAVVY resulted in a response having all the states where employees worked, due to the matching of ``IN" with the state code for Indiana.
Another methodology employs syntax-based systems. An example of this kind of system is LUNAR \cite{woods1973progress} where a syntactic parser generates a parse tree that is mapped using rules to an underlying database query language.
% These kinds of systems only work when the mapping from the parse tree to the query language is carefully designed keeping the database in mind. It is hard to scale and moreover hard to migrate to standard query languages or to other domains. 
A stricter grammar that takes into account the semantic categories instead of just syntactic are used in semantic-grammar systems such as \cite{thompson1969rel,waltz1978english,hendrix1978developing,templeton1983problems}. Building the parse tree in this type of setting involves having non terminal nodes as semantic categories which constrain the possible assignments to the tree in such a way that the mapping from the tree to the query language is easier. Although it streamlines the flow for a given task, this inclusion of semantic knowledge of a specific domain makes it even harder to adapt to other domains. This is in contrast to the syntax-based grammars where it is possible to at least re-use generic syntactic information across domains. An in depth compilation of the various NLIDB systems prior to the 90s can be found in \cite{androutsopoulos1995natural}.

% Following this, attempts to combine syntactic and semantic knowledge led \cite{rim1990transforming} to build a method for transforming syntactic graphs to semantic graphs

% Early semantic parsing systems used knowledge representation systems like KL-ONE and Loom. Parsing in \cite{psiklone} was done using a method described as "incremental description refinement" using a system called PSI-KLONE (Parsing and Semantic Interpretation in KL-ONE). 
% % These were unification based approaches not too different from some works even today which use search based techniques to grow the answers based on conditions that are satisfied \cite{mmrn}. 
% An early paper using this type of process \cite{kasper1990performing} attempts to merge unification based parsing with classification based knowledge representation. This method assumes that the model has access to a lexical analyzer that gives type membership information for each word. It also assumes the availability of a context free grammar that is able to assign grammatical functions to the words. An initial description is given to the classifier which then uses lattice representations of the defined types to guide the search in the space of types that are satisfied by a given object. The authors showed that this classification based parsing method overcame several sources of inefficiencies that are inherent in the unification based models. However, the method relies heavily on access to the language feature descriptions. Another work around the same time \cite{rim1990transforming} deals with the principle that ambiguity is an intrinsic property of natural language. They compute a syntactic graph and an exclusion matrix using an all paths chart parser. The authors then transform these into a functional graph which after further processing gives the semantic graph. For example, by using the graph and matrix in Figure \ref{fig:sem_graph}, questions such as "Does the monkey live in jungles?", "Where does the monkey live?" can be answered directly from the graph by matching paths from the question through the graph while maintaining that none of the arcs in the answering path co-occur with any other. Essentially, this method was more efficient than previous attempts to just use semantic filtering rules because once the rule rejects a particular relation, it is possible to exclude many syntactic representations from further consideration by pruning all dependent relation of that relation from the semantic graph. 
\subsection{Rise of statistical techniques}
The seminal work of \citet{zelle1996learning} introduced a model which is able to train on a corpus of pairs of sentences and database queries. The system employed a deterministic shift reduce parser and developed an algorithm called \texttt{CHILL} which is based on Inductive Logic Programming.
% which works by learning control rules for parsing. Explain ILP?
% During parsing, the current context is maintained in a stack and a
% buffer contains the remaining input. When parsing is complete, the stack contains the representation of the input sentence. 
% This is in contrast to the previous methods of the time that relied on hand crafted rules. 
The previous work that had used corpus based training were all focused on shallow parsing, using corpora that had to be previously annotated with syntactic information.
% (with the usage of lexical analyzers that gives type membership information for each word).
The evaluation of these systems was also imperfect as they were compared based on simulated metrics of parsing accuracy. On the other hand, \citet{zelle1996learning} build a framework which converts the natural language sentence to a database query, facilitating straightforward evaluation: by implementing the query on the database, one can check if the answer returned is satisfactory. The operators used in this framework require a semantic lexicon as a-priori knowledge. \citet{thompson2003acquiring} improve on this by learning a lexicon of phrases paired with meaning representations, from the data. Experimental results showed that a parser using the learned lexicon performs comparably to one that uses a hand built lexicon. This data driven approach also allowed lexicons and parsers to be easily built for multiple languages --- Spanish, Japanese and Turkish. 
However, even \citet{zelle1996learning} required annotated examples where the annotation effort is not trivial. To help with this, \citet{thompson1999active} suggest looking at alternative training procedures which involve using active learning in order to reduce the number of annotated examples required to solve complex tasks. 
% This is accomplished by either \textit{constructing} examples, procuring certain \textit{types} of examples or by trying to figure out which examples from a given set of unsupervised examples are the \textit{most useful}.
% In the case of natural language where we have at our disposal plenty of text, it would be most profitable if we could focus efforts on only annotating the sentences that give us the most \textit{information}. They use certainty based selective sampling whereby the model is trained on a small number of annotated examples to learn the preliminary classifier. On subsequent examination of un-annotated examples, the system assigns certainties to the predicted annotation of these examples. The k samples that have the lowest certainties are given to the user for annotation and retraining. The certainty assignment can be done in multiple ways but is typically implemented by calculating the probability that a classifier that is consistent with the earlier training data would have classified new examples appropriately.

% A model trained on very few examples would overfit to the examples it has seen and would be unable to complete the parse of the new sentence. This can either occur because the control rules learned for an operator might be too specific, or because the operator that is needed for parsing this new sentence was unseen previously and hence not included as a possible action. The uncertainty in these incomplete parses would certainly be high and hence the authors come up with a different metric to measure this uncertainty. They count the maximum number of operators successfully applied during the process of generating the parse and divide that by the number of words in the sentence to get a value for how close the parser came to completing the parse. The lower values sentences are then given higher priority for annotation. They conducted experiments on the Geo880 data set which enables comparison with the earlier \cite{zelle1996learning} model. The authors found that the gains were not significant at less number of training examples, but after 100 examples, the active learned model is better. They report that to reach within 5\% of the final accuracy, only 125 selected examples are needed as opposed to 175 randomly sampled examples (savings of 20\%). In Figure \ref{fig:active}, Geobase refers to the hand built benchmark and we see that the active learned model requires less than 100 selected examples as opposed to 125 random examples to beat this baseline. 




% In 2001, \cite{tang2001using} tried a different approach for learning whereby they combined different learning methods in Inductive Programming Logic allowing a learner to be more expressive than would be possible using the individual learners. This is especially useful in cases where the performance on the task relies on figuring out a variety of classification problems, each of which have their own peculiarity which may or may not suit certain learning methods. 

A consistent theme through these times was the increasing use of statistical learning techniques that are able to learn models on given examples of desired input output pairs. Among the fully supervised attempts at semantic parsing using fully annotated sentence-logical form pairs are \cite{zelle1996learning,zettlemoyer2005learning,zettlemoyer2007online,kwiatkowski2010inducing}. In \citet{zettlemoyer2005learning}, the learning algorithm takes as input pairs of sentences and their respective lambda-calculus expressions. An example of this kind of pair from the GeoQuery domain is :  \texttt{What states border Texas} :$\lambda x.state(x) ∧ borders(x, texas)$.
Given a CCG lexicon L, there would be many different parses that could result for a given sentence. To deal with this ambiguity, a PCCG (Probabilistic CCG) defines a method for ranking possible parses
for a given sentence in terms of the probability. More concretely, a log linear model that is characterized by a feature vector \textit{f} and a parameter vector $\theta$, is usually used to select the most likely parse. For a given sentence \textit{s}, parse \textit{z} and logical expression \textit{l}, the log linear model is defined as :
\[ P(z,l|s;\theta,L) = \frac{e^{\theta f(s,z,l)}}{\sum_{(z',l')}e^{\theta f(s,z',l')}}
\] 
The features could be as simple as counts of certain lexical entries in the current parse. The parsing (inference) part of the process involves finding the most likely logical form \textit{l}, given an input sentence \textit{s} when the parameters and the lexicon are known: 
\[F(x) = \arg\max_{l} p(l|s;\theta,L) 
= \arg\max_{l} \sum_{z} P(z,l|s;\theta,L)
\]
obtained by marginalizing over all the latent parses \textit{z}.
If the feature vectors only operate locally, it is possible to employ dynamic programming approaches such as those employed in CKY parsing algorithms used for finding the most likely parse in probabilistic context free grammars \cite{manning1999foundations}. Beam search is used during parsing to remove low probability parses, increasing efficiency. 

% The model provides a CCG along with parameters for a log linear distribution over parses that  satisfy the grammar, without using any auxiliary information such as parse trees.
In \citet{zettlemoyer2005learning}, the lexicon is induced as part of the learning procedure by only preserving lexical entries that result in the required parse.
However such a system would have issues due to the inflexibility of CCG when it is applied to raw natural language inputs, having variable ordering of words, colloquial language and sometimes even missing words.
\citet{zettlemoyer2007online} tweak the learning algorithm so that it is possible to deal with these kinds of variations.
% that would be otherwise hard to deal with using strict grammars.
This is carried out by using extra combinators that are not standard CCG, by relaxing some parts of the grammar such as the ordering of words along with having learned costs for these new operations.
They also describe a novel online algorithm for CCG learning which employs perceptron training of a model with hidden variables, while also inducing grammar in an online fashion.
Meanwhile, \citet{kwiatkowski2010inducing} aim to have a more general framework that is agnostic to the choice of natural language as well as logical expressions, using a CCG, followed by higher order unification which allows the model to search the space of all grammars consistent with training data, while also allowing estimation of the parameters for the log-linear parsing model. 
% Higher order unification, in the context of this work, refers to finding substitutions for the free variables in a pair of lambda calculus expressions that result in equivalent expressions.
% They are still unable to handle unedited sentences that are noisy and challenging. Work by \cite{kwiatkowski2011lexical} improves upon this, as explained next. 


% paved the way for learning semantic parsers from pairs of sentences and meaning representations using algorithms for learning probabilistic CCG grammars,
However, \citet{zettlemoyer2005learning, zettlemoyer2007online}
 had deficiencies in the form of data sparsity caused by not sharing weights for related classes of words. \citet{kwiatkowski2011lexical} improve upon this by introducing factored lexicons.
%  where it is no longer necessary to build up a lexicon having multiple lexical entries with different syntactic contexts, but differing only in the constants. 
 The main intuition behind this work is that within a particular class of words, the variation between the lexical items is \textit{systematic}. Decomposing the lexical entries allows sharing of information between multiple lexical entries, easing the issue of data sparsity. 
They address this by splitting the lexicon into \textbf{lexemes} which are mappings from natural language words or phrases to a set of logical constants and \textbf{lexical templates} which are pre-defined templates used to capture the variable usage of words. 
This decomposition results in a more concise lexicon which also requires less data to learn from. Subsequent work using CCGs mostly employ this factored lexicon approach. 

A consequence of the fact that these systems require complex annotation is that they are hard to scale and they only work in narrow domains.  Generating the data sets using manual annotation is still a formidable task and due to this, supervision in various different forms has been explored. The next two sections list several of these attempts.

==> Semantic parsing survey/sections/from_denotations.tex <==
The next transition came from training systems solely on the \textbf{result} of the execution (a.k.a. denotation) of the formal meaning representation (program), in the absence of access to the program itself. This can take many forms, e.g. the result of executing a query on a KB, the final state of a robot that is given instructions, etc. 
% This allowed building data sets that were an order of magnitude larger than those of the time due to the ease of generating these data sets by crowd sourcing.
Training models with such \textbf{weak supervision} poses certain challenges. The first is an extremely \textbf{large space} of potential programs that have to be explored during training. The second is the noise that is inevitable in these systems due to \textbf{spurious programs} that lead to the correct answer by chance. 

% Question answering can be broadly divided into structured semantic parsing based QA involving mapping of a question to a meaning representation that is executed on a knowledge base, versus unstructured QA where a question is answered directly from some text. The meat of the problem for semantic parsing based QA lies in understanding the question which can have multiple compositions. On the other hand, unstructured QA \cite{das2017question,chen2017reading,wang2018r3,sun2018open}  mainly focuses on the retrieval task of matching queries to documents and then obtaining the answer using some local context such as the paragraph or sentence that is retrieved. In this survey, we will focus on the first kind. 

\citet{berant2013semantic} learn a semantic parser from question answer pairs on Freebase. A major problem while using such large KBs is that there exist a very large number of logical predicates for a given question. They use a two step process to deal with this issue: they first have a coarse grained solution by aligning the sentences to predicates of the KB by asserting that a phrase and a predicate align if they co-occur with many of the same entities. They then have a bridging operation which provides additional predicates by looking at the neighbors. This is especially helpful when the predicates are expressed weakly or implicitly. 
% Similar to \cite{liang2011learning} and \cite{zettlemoyer2005learning}, a log linear model over all the possible derivations that result given a specific input utterance is learned using MML. (\S~\ref{sec:mml}). 
Concurrent work by \citet{kwiatkowski2013scaling} also employs a two stage approach which involves first using a CCG to map utterances to an abstract under-specified form which is domain independent. This abstraction allows sharing across different domains (\S~\ref{sec:intermediate}), instead of having to learn the rules for each target domain. This is followed by an ontology matching step wherein the domain specific knowledge is incorporated using information about the target ontology as well as lexical similarity between constants that are part of the under specified form and the domain specific constants.
A linear model over all derivations is learned, involving the CCG parsing steps as well as the ontology matching, with supervision only in the form of final answers to the questions. 

\citet{pasupat2015compositional} use question-answer pairs as supervision to tackle the task of answering complex questions on semi-structured tables. They use a realistic setting where the train and test tables are disjoint so that the model should be able to generalize to entities and relations that were not seen at training. A consequence of this is that the regular approach of building a lexicon with mappings from phrases to relations cannot be built and stored. Further, due to the complex nature of the questions that involve operations such as aggregations and comparisons, the search space of all possible logical forms grows exponentially. To combat the issue with the unseen tables, their approach first builds a knowledge graph from the table in question resulting in an encoding of all the relevant relations. Using the information from this graph, candidate parses of the question are generated and these candidates are ranked using a log linear model, whose parameters are learned using MML (\S~\ref{sec:mml}). To deal with the exploding search space, they use beam search with strong type and denotation constraints along with strict pruning of invalid or redundant logical forms. 

In the context of semantic parsing for robot navigation, the training data consists of triples of a natural language instruction, start state and validation function that specifies whether the set of actions produced the expected result. \citet{artzi2013weakly} use a grounded CCG by incorporating the execution of the logical form in each state to drive the CCG parsing. This joint inference procedure allows the parser to leverage cues from the environment, making it possible to learn while executing the instructions. 

% \citet{clarke2010driving} employ binary feedback signals to direct learning in another attempt at training a semantic parser from denotation. The feedback essentially checks whether the response after executing the query on the database was satisfactory. They use Integer Linear Programming, allowing them to introduce some domain knowledge into the inference process and thereby restricting the space of possible results. A major strength of their approach is that they are able to deal with various syntactic variations of the same meaning representations without extra effort as was required in \cite{zettlemoyer2007online}.
% \citet{iyer2017learning} also use a similar feedback mechanism in order to develop their training set. They operate in an online setting where they use binary feedback from the user to decide if a particular input-output pair should be added to the training set or if it should be sent to the crowd sourced workers for re-annotation. This approach allowed them to reduce the annotation effort over time as the model trains and provides better results.

==> Semantic parsing survey/sections/indirect_supervision.tex <==
% \subsection{Auxiliary syntactic information}
\noindent \textbf{Auxiliary syntactic information}:
\citet{krishnamurthy2012weakly} are able to train a semantic parser without needing any sentence-level annotations. Instead, they combine readily available syntactic and semantic knowledge to construct a versatile semantic parser that can be applied to \textit{any} knowledge base. Using just the knowledge base and automatically dependency parsed sentences from a web corpus, they are able to generate the correct logical form with 56\% recall. Using dependency parse based heuristics, a lexicon is generated for relation instances that occur in the web based corpus. A mention identification procedure links these to entities in the knowledge base resulting in triples consisting of sentences, along with two identified mentions. By matching the dependency path between the two entity mentions to a set of pre-identified patterns, lexical entries are generated. This lexicon is used by the CCG parser with allowances to skip words that do not occur in the vocabulary of the knowledge base --- ensuring that the logical forms contain only predicates from the knowledge base. The resulting parser is able to handle complex constructs having conjunctions of various categories as well as relations that share arguments. 

% Their model works by finding relation instances directly from the knowledge base while at the same time maintaining the constraint that the parse generated also satisfy the dependency parses. The authors are even able to discover richer semantic structures by using this method, such as those obtained as a result of conjunctions of multiple relations. This method which is essentially simple string matching can capture verbs, common nouns such as "city", noun compounds "New York city" and much more.
% The model uses a corpus of dependency-parsed sentences with a CCG lexicon and produces logic forms containing predicates from the knowledge base. It uses a simple string matching technique for identifying entities in sentences from the knowledge base. Since the correct logical form for each sentence is not previously observed, the proposed model uses weak supervision in the form of constraints. First  every relation $r(e_1,e_2) \in \Delta$ in the knowledge base should be expressed by at least one sentence in the training data. Second, the correct semantic parse of a sentence contains a subset of the syntactic dependencies contained in a dependency parse of that sentence. The output of this model are parameters $\theta$ for the CCG which produce the correct semantic parse for sentences in the training data. 
\noindent \textbf{Unsupervised}:
% \subsection{Unsupervised}
\cite{poon2009unsupervised} was the first attempt at learning a semantic parsing model in an unsupervised manner. They begin by clustering tokens that are of the same type, followed by recursively combining sub-expressions that belong to the same cluster. Their model learns to successfully map active and passive voices to the same logical form showing the robustness of their approach. 
They evaluate their model on a fact prediction task on a KB that they extract from the GENIA \cite{kim2003genia} biomedical corpus. A major problem with the approach of generating self induced clusters for the target logical forms is the mismatch with existent ontology and databases. As a result, their approach is unable to answer complex questions on existing databases without an extra ontology matching step.
% for resolving the clusters with elements of the database.
Instead, \citet{poon2013grounded} exploit the database as a form of indirect supervision, allowing them to attack more complex questions. Here, they combine the unsupervised semantic parsing approach with grounded learning using the database. A probabilistic grammar is learned using EM and the main merit of their method is that the search space is constrained using the database schema making learning much easier and also ensures that the parses that are generated can be readily executed on the database. 

\noindent\textbf{Supervision from conversations}:
An unusual source of supervision for semantic parsing systems is from conversations. \citet{artzi2011bootstrapping} use conversational feedback in order to learn the meaning representation for user utterances. They induce semantic parsers from un-annotated conversational logs. They posit that it is often possible to decipher the meaning of an utterance by analysing the dialog that follows it. They use a PCCG  for inducing the grammar and by using a loss sensitive perceptron algorithm, the model obtains a rough estimate of how well a possible meaning for an utterance matches with what conversation followed after it as well as how much it matches our expectations of what is generally said in the dialog's domain.
% Using this loss function, both the parameters of the PCCG as well as the lexicon generation are learned. 

\noindent\textbf{Visually grounded semantic parsing}:
Recent work by \citet{videocaption} involves learning a semantic parser using captioned videos. Using a factored lexicon approach as in  \cite{kwiatkowski2011lexical}, they employ a weighted linear CCG based semantic parser that uses supervision in the form of a visual validation function. This function provides a sense of the compatibility of a parse with a given video and is the only supervision used to drive the lexicon generation process in the modified GENLEX \cite{artzi2013semantic}. While the parser is learned using the videos, they are not used at test time. 

\noindent\textbf{Using canonical forms}:
\label{sec:canonical}
\citet{wang2015building} demonstrate how to train a semantic parser in a domain starting with zero training examples. Their framework has two parts - the first is a \textit{builder} that provides a seed lexicon containing a canonical form for each predicate, given the target database schema. The second part is a \textit{domain general grammar} that uses predicate-canonical form pairs from the seed lexicon to generate pairs of logical expressions and \textit{canonical utterances}, which are ill-formed natural language-like sentences preserving the semantics of the corresponding logical expressions. Crowd workers are then employed to paraphrase these canonical utterances to actual natural language utterances to build the data set. 
This method has the advantage of being \textit{complete} in the sense that the entire logical functionality of the grammar is reflected in the data set due to the reverse way in which it is built. This is in contrast to other approaches where the questions and answers in the data set dictate the abilities of a semantic parser. For example, the WebQuestions dataset does not have any instances of questions with numerical answers, resulting in any semantic parser trained on this data set to also not be able to handle such cases. It is also an easier effort to generate annotations for paraphrases than actual answers to the questions, reducing the burden on the crowd worker and making the cost of the jobs lesser.\\
\noindent\textbf{Machine translation techniques}:
\citet{wong2006learning} employ statistical machine translation (MT) techniques for the task of semantic parsing by arguing that a parsing model can also be viewed as a syntax-based translation model. They achieve good performance and develop a model that is more robust to word order. The authors tried to depart from the more deterministic parsing strategies that were prevalent at the time \cite{zelle1996learning,kate2005learning} and
% They also neither use prior knowledge of the syntax nor do they use parse trees.
only assume access to an unambiguous, context free grammar of the target logical form. 
% The paper builds on the work by \citet{kate2005learning} in which the proposed model is able to induce transformation rules that convert natural language to a standard logical form. The model exploits the non terminal symbols in the formal grammar for the target logical form to learn the transformation rules. It incrementally converts the parse tree representation of the natural language to the parse tree representation of the output logical form. 
Building on the work by \cite{kate2005learning}, \citet{wong2006learning} use a statistical word alignment algorithm as seen in \cite{brown1993mathematics} in order to get a bilingual lexicon which has pairings of the natural language sentence with its respective translation in the logical form. The full logical form is obtained by combining all the input sub strings and their translations.
\citet{andreas2013semantic} explicitly model semantic parsing as a MT task and achieve results comparable to the state of the art on GeoQuery at the time. 
% They employ certain pre and processing steps that make it possible to impose the structure that is inherent to the meaning representation language(MRL).
In order to use MT techniques, they linearize the meaning representation language (MRL) by performing a pre-order traversal of each function and label every token with the number of arguments it takes, which is later used during decoding to distinguish well-formed MRs. It also helps to model functions that can take multiple number of arguments during alignment, depending on the context. 
% Many-to-many alignments are provided by an alignment algorithm which is then used to extract translation rules. 
Both phrase based and hierarchical translation models are used to extract pairs of source$\leftrightarrow $target aligned sentences. 
% To ensure more emphasis is given on well formed MRs, 
A language model is learned on the MR training data so that the model learns which arguments are more favoured by particular predicates of the MRL. The success of this work demonstrated that MT methods should be considered as competitive baselines.\\
\noindent\textbf{Learning from user feedback}: \citet{iyer2017learning} present an approach to improve a neural semantic parser based on user feedback wherein a rudimentary parser is used to bootstrap, followed by incorporating binary user feedback to improve the parse.
% They deploy a parser (trained initially using supervised learning to produce SQL queries) and show that it can be improved via incorporating user feedback. A user asks a question to the deployed system and the results of executing the predicted SQL query are presented to an user who provides a binary feedback. If the predicted answer is incorrect, then the user is asked to modify the predicted SQL query. This approach relies on the popularity of SQL and would be hard to apply it to existing systems that depend on a domain specific query language.
In \citet{lawrence2018improving}, the semantic parser is improved using interaction logs, available in abundance as a result of commercially deployed systems logging a huge amount of user interaction data, and employs a form of counterfactual learning \cite{bottou2013counterfactual}. They show improvements on the \textsc{nlmaps} dataset in the \textsc{OpenStreetMap} domain. 
% They design a special user interface for collecting user feedback on various facets of a question (such as location, question type, proximity). They also show significant improvement in a simulated log setting.
Although this work is specifically designed to work on a small system it a promising avenue especially for industry due to the extensive availability of logged data.



% using a frame word called synchronous CFG (context free grammar), as described in \cite{aho1972theory}.
% The algorithm is called ``WASP", Word Alignment-based Semantic Parsing. 
% The semantic parsing model is based on synchronous parsing, which was originally a theory of compilers wherein analysis of syntax and code generation were done in a single step. Given an input natural language sequence, the task is to find a derivation that produces a translation of the input. However, there are many possible derivations that could be generated for a given input. In this method, a set of derivations are generated and a choice is made among these by a model that maximizes the likelihood of the derivation given the input. The overall algorithm employs a two step process: first, a lexicon mapping from natural language to the logical form is learned by training  a statistical word alignment model on the training data consisting of pairs of natural language to meaning representation. The lexicon is constructed by using the K (set to 10) most probable transformations \cite{kate2005learning} from natural language to the meaning representation. This bilingual lexicon then has mappings from natural language sub strings to translations in the target meaning representation language. The final parse is then generated using synchronous CFG that can produce many possible derivations.  So to choose among these, the second step is to induce the probabilistic model to choose the correct derivation and subsequently the correct output translation. 



==> Semantic parsing survey/sections/intro.tex <==

% Explain contributions and show how different from Liangs document!!

An important area of research cutting across natural language processing, information retrieval and human computer interaction is that of natural language understanding (NLU). Central to the objective of NLU is semantic parsing, which is framed as a mapping from natural language utterances to meaning representations. The meaning representation thus generated goes beyond shallow identification of roles and objects in a sentence to the point where it enables automated reasoning. It can be executed in a variety of environments in order to enable tasks such as understanding and executing commands for robotic navigation, data exploration and analysis by parsing natural language to database queries and query parsing in conversational agents such as Siri and Alexa.

Further, it is worthwhile to recognize that semantic parsing is inherently different from other sequential prediction tasks such as machine translation and natural language generation in that unlike the latter, it involves prediction of inherently structured objects that are more tree-like. Additionally, it has to also adhere to certain constraints in order to actually execute in a given environment, introducing unique challenges.

% Depending on the type of output representation resulting from the system attempting to perform NLU, it can be categorized into various subtopics such as relation extraction, semantic parsing, sentiment analysis and building vector space models to understand topic distributions. 

% Semantic parsing in the context of building natural language interfaces to database (NLIDB) is extremely relevant in today’s world, where we have available large data stores and need efficient and robust methods to query them effectively.


% involves building natural language interfaces to computers. Semantic parsing frames this task as a mapping from natural language to a meaning representation, given a context. This representation goes beyond shallow identification of roles and objects in a sentence to the point where it enables automated reasoning. Semantic parsing is extremely relevant especially in the context of building natural language interfaces to database (NLIDB) in today's world, where we have available large data stores and need efficient and robust methods to query them effectively. 
% Another important advantage of NLIDBs is in the ability to handle anaphoric expressions. Systems based on conversational question answering attempt to work for brief, under-specified questions which are understood in the context of the preceding discourse. 

The contributions of this survey are firstly, to introduce the key components of the semantic parsing framework. Secondly, to make an uninformed reader comfortable with the field by providing an intuition for how it has developed through the years. Thirdly, to contrast various methodologies that have been followed in terms of the level of supervision, types of training strategies, amount of feature engineering and ways to incorporate structural constraints. 

To make a reader familiar with the terminology used, (\S~\ref{sec:term}) formally introduces the task of semantic parsing along with its fundamental components. In  (\S~\ref{sec:early}) we will explore the field from its early days where systems were based on hand crafted rules, restricting them to narrow domains and trace its path through times where we learned statistical models on examples of input-output mappings. 
% Statistical models are used to learn weights on candidate derivations and produce the final meaning representation. The constructed meaning representation is rendered as a \textit{logical expression} (sometimes latent to the derivation) that can be evaluated by executing on data held in various formats. 
The mapping to logical forms typically relies heavily on the availability of annotated logical forms and difficulties in procuring such labeled data gave rise to attempts at using alternative methods of training involving weak supervision.
 (\S~\ref{sec:qa}) describes the transition to using data sets that consist of questions annotated only with the final denotation, giving way to new styles of training.  (\S~\ref{sec:indirect}) details alternative forms of supervision. (\S~\ref{sec:enterseq2seq}) describes the adoption of encoder decoder frameworks to model the semantic parsing task. The three common learning paradigms used to learn the parameters of the model are explained in (\S~\ref{sec:learning}). 

% Important components of the semantic parsing framework are the language (or executor \cite{liang2016learning}) and grammar that are used to construct the logical form. We trace the field as it evolves from using lambda calculus \cite{church1985calculi}, combinatorial categorial grammars  \cite{ccg} and dependency-based compositional semantics \cite{liang2013lambda} to the current times where attempts are being made to convert the natural language question directly to user friendly languages like SQL with good database interfacing implementations. 

==> Semantic parsing survey/sections/learning.tex <==
% Learning consists of 
\subsection{Maximum marginal likelihood (MML)}
\label{sec:mml}
In the \textbf{fully supervised setting} where the training set consists of $\{(x_i, y_i, c_i) : i = 1 \ldots n\}$, with access to the natural language utterance $x_i$, the \emph{fully annotated output logical form} $y_i$ and the context $c_i$, this objective is of the form:
\[
J_{MML} = \log p(y_i|x_i, c) = \log \sum_{d\in D}p(y_i,d|x_i,c)
\]
where D is the set of all possible derivations that produce the logical form $y_i$. These are generated as part of the parsing procedure and are not available as part of the training set. These derivations are treated as latent variables and marginalized out of the objective. 

In the \textbf{weakly supervised setting}, when our training data is of the form \\$\{(x_i, z_i, c_i) : i = 1 \ldots n\}$, where $z_i$ is the denotation obtained after executing the latent logical form $y_i$ on the context $c_i$, the objective is of the form:
\[J_{MML} = \log p(z_i|x_i, c) = \log \sum_{y \in Y} p(z_i|y,c_i)p(y|x_i,c_i)
\] 

% Here, we assume the model is able to directly predict the output logical form without considering intermediate derivations $d$. 
In this case, we only need to check whether the denotation obtained as a result of the execution of a given $y$ $ \in Y $ (where Y is the set of all programs) on $c$ is equal to $z$. Depending on this, the first term of the summation is either a 1 or 0. Further, considering $Y^*$ as the set containing only the programs that execute to the correct denotation $z$ , we obtain the following:
\[J_{MML} = \log \sum_{y \in Y^*}p(y|x_i,c_i)\]

In practice, the set of y that are considered is usually approximated using beam search. The search space is typically pruned using strong type constraints. The search procedure can be done as part of the learning in an \textit{online} manner, or executed beforehand in an \textit{offline} manner, which we describe next. 
% \subsubsection{Online search}

\noindent \textbf{Online search} --- Several works in semantic parsing literature employ MML with online search \cite{pasupat2015compositional, liang2011learning, berant2013semantic, goldman2017weakly}. Including the search process as part of the learning necessitates running a beam search with a wide beam (for example $k$=500 in \cite{berant2013semantic}), leading to expensive back propagation updates. The set of candidate logical forms keep changing in this approach and there is still no guarantee that every logical form that executes to the correct denotation will be included in the beam. 

% \subsubsection{Offline search}
\noindent \textbf{Offline search} --- In this setting, a set of logical forms that result in the correct final denotation are automatically generated beforehand for each example. \citet{krishnamurthy2017neural} use this procedure referred to as \textit{dynamic program on denotations} (DPD)\cite{pasupat2016inferring}, which leverages the fact that the space of possible denotations grows much more slowly than that of logical forms, since many logical forms can have the same denotation. This enumeration makes it possible to have smaller beam sizes as a result of collapsing together many logical forms which have the same denotation. Further, DPD is guaranteed to recover all consistent logical forms up until some bounded size.


\subsection{Reinforcement learning}
In this learning paradigm, an agent is considered to make a sequence of decisions based on a policy and receives a reward $R(y,z)$ for a given program $y$ and answer $z$ at the end of the sequence if the sequence executes to the correct denotation z, and 0 otherwise. Typically, a stochastic policy is trained with the goal of maximizing the expected reward. 
The expected reward for an example $(x_i,z_i,c_i)$ can be written as:
\[ J_{RL} = \sum_{y \in Y}p(y|x_i,c_i)R(y,z_i) \]
Since the set of all possible programs is large, the gradient is computed by sampling from the policy distribution.
This is problematic when the search space is large and special techniques are employed to improve sampling. \cite{liang2016neural,zhong2017seq2sql,andreas2016learning,misra2018policy, das2017go}.

An issue with both of the above approaches is that they are based on exploration as a function of the model's current policy. This means that if a correct program is incorrectly assigned a low probability, it will fall out of the beam, or in the RL version, not be further sampled, further down-weighting the probability of this program. The same applies for falsely high probability \textit{spurious} programs that incorrectly gain even more importance. Further, the REINFORCE \cite{williams1992simple} method has the added disadvantage that in the case of peaky distributions, i.e., a single program accounts almost entirely for the probability under the current policy, it will repeatedly sample the mode of the distribution. On the other hand, MML based exploration using beam search will always use the N-1 spaces in its beam to explore programs other than the highest scoring one.  


\cite{guu2017language} demonstrate how to overcome this issue by suggesting an $\epsilon$-greedy randomized beam search that gets the best of both worlds. In this approach, they follow regular beam search to compute all possible continuations and rank them in descending order according to their probabilities. But, instead of just picking the top $k$ highest scoring continuations, they are uniformly sampled without replacement with probability $\epsilon$ and retrieved from the remaining pool according to their rank, with probability $1-\epsilon$. 
In a more principled approach to solving the exploration problem while also ensuring good sample efficiency, \citep{liang2018memory} propose a method that employs an external memory buffer that is used to keep track of high reward trajectories. They propose to also pick trajectories by rejection sampling using the memory buffer in addition to sampling from the buffer. This ensures that while high reward trajectories are not forgotten, it avoids giving too much importance to possibly spurious high reward trajectories, hence reducing the bias. Further, by keeping track of the high reward trajectories using the memory buffer, they are able to achieve a reduction in variance of the estimates by a factor that depends on the size of the buffer. They are able to outperform the previous state of the art on WikiTableQuestions. 

\subsection{Maximum margin reward methods (MMR)}
In this third learning model, training usually involves maximizing a margin or minimizing a risk. Similar to the latent variable structured perceptron \cite{zettlemoyer2007online} and its loss sensitive variants, this training paradigm involves structured output learning. Given a training set $\{(x_i, z_i, c_i) : i = 1 . . . n\}$, this method first finds the highest scoring program $y_i^*$ that executes to produce $z_i$ from the set of programs returned by the search.
Considering $y^*$ is the highest scoring program, we can find the set of all violating programs as:
\[ V = \{y'|y'\in Y \textrm{and }score_{\theta}(y^*,x,c) \leq score_{\theta}(y',x,c)+\delta(y^*,y',z)\}
\]
where the margin $\delta(y^*,y',z) = R(y^*,z)-R(y',z)$. From this, we obtain the most violating program as 
\[ \overline{y} =\argmax_{y' \in Y}\{score_{\theta}(y',x,c)-score_{\theta}(y^*,x,c)+\delta(y^*,y',z)\}
\]
So for a given example $(x_i, z_i, t_i)$ the max margin objective or negative margin loss as:
\[ J_{MMR} = - max\{0, score_{\theta}(\overline{y_i},x_i, t_i)-score_{\theta}(y_i^*,x_i,c_i)+\delta(y_i^*,\overline{y_i},z_i) \}
\]
Where only the score of the highest scoring program and the one that violates the margin the most, are updated. \citet{iyyer2017search} and \citet{mmrn} use this type of framework.
\citet{misra2018policy} explain how these various training paradigms relate to each other and provide a generalized update equation making it easier to choose an approach that would best suit a particular problem.

==> Semantic parsing survey/sections/seq2seq.tex <==
Over the last couple of years, there has been a rise in end to end approaches for semantic parsing using encoder-decoder frameworks based on recurrent neural networks. This approach has been largely successful in a variety of tasks such as machine translation \cite{kalchbrenner2013recurrent, cho2014learning, sutskever2014sequence}, syntactic parsing \cite{vinyals2015grammar}, image captioning \cite{vinyals2015show}, etc.  In the case of semantic parsing, it consists of learning a mapping from the natural language utterance to the meaning representation, avoiding the need for intermediate representations. This flexibility has advantages as well as disadvantages- it alleviates the need for defining lexicons, templates and manually generated features, making it possible for the models to generalize across domains and meaning representation languages. However, traditional approaches are able to better model and leverage the in-built knowledge of logic compositionality. 
\vspace{-0.70mm}

\citet{dong2016language} set this up as a sequence transduction task where the encoder and decoder are in the same format as defined by \citet{sutskever2014sequence}, employing L-layer recurrent neural networks (LSTMs in this work) that process each token in the sequence. In order to better model the \textbf{hierarchical structure} of logical forms and make it easier for the decoder to keep track of additional information such as parentheses, the authors propose to use a decoder that takes into account the tree structure of the logical expression. This is enforced by having an action (a special token) for generating matching parentheses and recursively generating the sub-tree within those parentheses. The decoder is provided with additional \textbf{parent feeding connections} which provides information about the start of the sub-tree, along with soft attention to attend over tokens in the natural language utterance as in \citet{bahdanau2014neural} and is able to perform comparably against previous explicit feature based systems.
% Next, Section \ref{sec:seq2seq1} discusses issues regarding infrequent words and how to combat them. Section \ref{sec:intermediate} examines techniques where mapping to an intermediate representation allows the model to focus its capacity on capturing the abstract meaning of the utterance and later fill in the finer details. When the grammar of the target language is known, explicitly incorporating it into the decoding process is convenient, so that only actions that respect the underlying grammar can be taken. Section \ref{sec:seq3} discusses work that employs this type of approach. 

A fundamental concern regarding these methods is their inability to learn good enough parameters for \textbf{words that are rare} in the dataset. The long tail of entities in these small datasets raises the need for special pre-processing steps. A common method is to \textbf{anonymize the entities} with their respective types, given an ontology. For example towns such as Amherst are anonymized as \texttt{Town}, and later post processed to fill in the actual entity. Another approach to counter this is to use Pointer Networks \cite{vinyals2015pointer} where a word from the input utterance is directly copied over to the output at each decoding step. A combination of these two referred to as \textbf{attention-based copying}, allowing for more flexibility so that the decoder can either choose to copy over a word or to pick from a softmax over the entire vocabulary is employed in \cite{jia2016data}. This work also introduces an approach which can be classified as a data augmentation strategy. They propose to build a generative model over the training pairs (natural language to logical expression) and sample from this to generate many more training examples, including those of increased complexity. The model used to do the actual parsing task is the same as in \cite{bahdanau2014neural} and the main contribution of this work is the emphasis on a conditional independence property (which holds most of the time) that is fundamental to compositional semantics- \textit{the meaning of any semantically coherent phrase is conditionally independent of the rest of the sentence}. This allows them to build a synchronous context free grammar (SCFG) which the generative model samples from, to provide a distribution over pairs of utterances and logical expressions. We refer the reader to \cite{jia2016data} for more details on the grammar induction steps. This approach boosts performance, due in part to the more complex and longer sentences that are generated as part of the data recombination procedure, forcing the model to generalize better. 

% A way to address the issue of data scarcity is the semi supervised approach of \citet{kovcisky2016semantic} in which they treat the natural language utterance \textit{x} as latent and learn an autoencoder to reconstruct the logical expression \textit{y}. Essentially, it is a mapping \textit{y $\rightarrow{x} \rightarrow{y}$}, where the model is trained to reconstruct the logical expression. The model consists of two sequence to sequence models chained together. To overcome the inability to back propagate through discrete draws of symbols for x while training, the authors propose to model a token \textit{$x_t$} to be a distribution over the vocabulary of \textit{x}, drawn from a logistic-normal distribution. The parameters of this distribution for each time step are provided by the LSTM attending over the encoders output for that time step. Their setup allows them to train either in an unsupervised or supervised setting by appropriately altering the loss function - either a KL divergence term used to regularize the latent distribution over \textit{x}, or in the supervised case a reconstruction loss on (\textit{x},\textit{$\hat{x}$}) in addition to the common reconstruction loss over (\textit{y},\textit{$\hat{y}$}). They experiment with a weighted combination of the two for the semi-supervised setting and show gains in accuracy over the fully supervised setting. Note that \cite{jia2016data} and \cite{kovcisky2016semantic}, both explicitly utilize \textbf{knowledge of the grammar} as part of their model, by using the grammar to augment the data by generating more examples.
% % raj

\subsection{Employing Intermediate Representations}
\label{sec:intermediate}
In closed domains, learning mappings from lexical items to all program constants becomes cumbersome and introducing a degree of indirection has been shown to be beneficial. Disentangling higher and lower level semantic information allows modelling of meaning at varying levels of granularity. This is profitable as the abstract representation is more likely to generalize in examples across small data sets. Further, using this abstraction helps to reduce the search space of potential programs as well as the number of false positives that are generated due to spurious programs that can generate the same denotation (answers or binary labels) just by chance. 
    
Although frameworks based on the encoder decoder framework provide greater flexibility, they generally do not allow interpretation and insights into meaning composition. A two stage approach such as that employed by \citet{cheng2017learning} aims to build intermediate structures that provide insight into what the model has learned. Further they use a transition based approach for parsing which allows them to have non-local features - an advantage over other methods using chart parsing which require features to be decomposed over structures in order to be feasible.  

\citet{goldman2017weakly} utilize a fixed KB schema to generate a smaller lexicon that maps the more common lexical items to typed program constants. Here, due to the abstract representation being confined to the domain of spatial reasoning, they are able to specify seven abstract clusters of semantic types. Each of these clusters have their own lexicon having language to program pairs associated with the cluster. A rule based semantic parser then maps the abstract representation created to one of the manually annotated examples, if they match. To counter the limited applicability as a result of the rule based parser, the authors propose a method to augment their data by automatically generating programs from utterances by using manually annotated abstract representations. In this way, they can choose any abstract example and then instantiate the clusters that are present in it by sampling the utterance to program pairs which are in that abstract cluster. These generated examples are used to train a fully supervised seq2seq semantic parser that is then used to initialize the weakly supervised model. 
% Their method is very successful with reported gains of 14.8\% absolute accuracy. . 

A strong merit of these lifted intermediate representations is that they allow \textbf{sharing between examples}, leading to easier training. Similar methods to generate intermediate templates have been employed in  \cite{dong2018coarse} where a \textit{sketch} of the final output is used for easier decoding. These methods have the added advantage of having an idea of what the intended meaning for the utterance is at a high level, and can exploit this \textbf{global context} while producing the finer low level details of the parse. 

\subsection{Decoding using a constrained grammar}
\label{sec:seq3}
By explicitly providing the decoder with constraints in the form of a target language syntax, \citet{yin2017syntactic} alleviate the need for the model to discover the intrinsic grammar from scarce training data. The model's efforts can then be better concentrated on building the parse, guided by the known grammar rules. The natural language utterance is transduced into an Abstract Syntax Tree (AST) for a given programming language which is then converted to the programming language deterministically. Generation of the AST takes place through sequential application of \textit{actions}, where the set of possible actions at each time step incorporates all the
information about the underlying syntax of the language. \citet{xiao2016sequence} similarly employ the grammar model as prior information so that the generation of derivation trees is constrained by the grammar. By explicitly ensuring that the decoder's prediction satisfy \textit{type constraints} as provided by a type-constrained grammar, \citet{krishnamurthy2017neural} are able to perform significantly better than the Seq2Tree model from \cite{dong2016language} showing that it is not enough to just generate well-formed logical expressions, but having them satisfy type constraints is also important. 
They also employ entity linking to better map the question tokens to entities that they refer to. By using features such as NER tags, edit distance and lemma matches, they are able to better handle the problem of rare entities, for which it is difficult to learn good embeddings.
% However, this process can be expensive when the number of entities is very large and the authors suggest that certain low precision filtering techniques to identify subsets of entities of interest by using string overlap or similarity heuristics could be fruitful as a preliminary step. 

% \cite{neelakantan2016learning} 

\subsection{General Purpose Code Generation}
\label{sub:code_gen}
\textbf{Data.} Training such models requires a parallel corpus of natural language utterances and their corresponding PL form. Although such data sources are not readily available, one can employ distant supervision techniques to existing open source code bases (e.g. \texttt{github}\footnote{\url{http://github.com}}) and forums (e.g. \texttt{StackOverflow}\footnote{\url{http://stackoverflow.com}}) to gather such aligned data. For example, natural language descriptions can be mined from code comments, documentation strings (docstrings), commit messages, etc and can be aligned to the code. \citet{ling2016latent} introduced two datasets by aligning the open-source Java implementation of two trading card games -- \textsc{hearthstone} and \textsc{mtg} to the description in the playing cards. Similarly, \citet{barone2017parallel} develop a large dataset of Python functions aligned to their docstrings and \citet{iyer2018mapping} introduce the \textsc{concode} dataset where both method docstrings and an initial snippet of code context is aligned to the implementation of a method in a Java class. 
% Open source programming forums such as \texttt{StackOverflow} also serve as a great resource.
Other datasets are introduced in \cite{iyer2016summarizing,yao2018staqc,lin2018nl2bash, oda2015learning}. 
% For example, \citet{iyer2016summarizing} introduce a dataset with automatically aligned question code pairs and \citet{yao2018staqc} introduce a human-annotated dataset of  question code pairs with a label indicating if the question can be answered with the code snippet alone. Recently, \citet{lin2018nl2bash} introduced a human-annotated dataset of aligned english sentences to one-liner Bash commands. \citet{oda2015learning} aims to learn to generate pseudocode from code and also introduced the \textsc{django} dataset that has aligned pseudo-code and code pairs. 

% There also exists some small datasets which were designed for a specific application and contains aligned natural language utterances with SQL queries. Notable examples are \textsc{Atis} \cite{price1990evaluation,dahl1994expanding} for flight booking, \textsc{GeoQuery} \cite{zelle1996learning} for user queries about US geography, \textsc{Restaurants} \cite{tang2000automated} for user queries about restaturants, their food types and locations and more recently the \textsc{scholar} dataset \cite{iyer2017learning} for user queries about academic publications.

    \noindent \textbf{Methodology.} Most contemporary works design the problem of code generation in the encoder-decoder (seq2seq) framework. The various datasets have their idiosyncracies, e.g. SQL and Bash datasets are generally single line of source code and hence the target sequence is short in length. On the contrary in \textsc{hearthstone} and \textsc{mtg}, models have to generate an entire class structure given the natural language description. 

The encoder module is usually a variant of bidirectional recurrent neural network architecture where the input consists of word level tokens \cite{yin2017syntactic} or characters \cite{ling2016latent}. The encoder module of \citet{rabinovich2017abstract} takes advantage of the structure present in the input (e.g. various textual fields of each cards in the \textsc{hearthstone} dataset) and encodes each component separately. 

Since PLs have a well-defined underlying syntax, the decoder module presents more interesting challenges. Initial work by \citet{ling2016latent} ignores any such syntactic constraints and lets the model learn the syntax from data. As a result, there is a possibility they may produce syntactially ill-formed code. Later work by \citet{yin2017syntactic}, \citet{rabinovich2017abstract} and \citet{iyer2019learning} explicitly model the underlying syntax of the PL in the decoding stage and hence can guarantee well-formed code.
% \citet{yin2017syntactic} has been described in \S~(\ref{sec:seq3}).
Similarly, \citet{sun2018semantic} develop a model which explicitly encodes the table structure and SQL syntax for the task of sequence to SQL generation. In \citet{rabinovich2017abstract}, the decoder module decomposes into several classes of modules and these are composed to generate the \emph{abstract syntax trees} (ASTs) in a top-down manner. 
% Explicit modules are defined for each grammar constructs, e.g. there are modules for both primitive and composite types. For each composite type, there are submodules for each of the constructor types and further each field of constructors are associated with their own modules. 
Learning corresponds to learning the sequence of decisions and is guided by the ASTs during training. This work can be seen as complimentary to neural module networks \cite{andreas2016neural,andreas2016learning,hu2017learning}.

% \raj{TODO: Please think about a table schema to place all this dataset compactly in a table}

% \subsection{Context}
% \subsection{Dialog systems}


% \cite{reddy2014large} provide a method for training a semantic parser using neither annotated logical pairs, nor question answer pairs. They assert that semantic parsing is essentially a graph matching problem. They convert an open domain CCG parsers output into a graph which is then grounded using a knowledge base. The grounding is done by mapping the graph that is generated from the CCG with all the possible sub graphs from Freebase (nodes and edges mapped to types and relations respectively). However, the problem arises that there can be multiple grounded subgraphs to choose from, and to tackle this they use weak supervision in the from of similarities between denotations of natural language queries and their related Freebase queries.

% \cite{yih2015semantic} extend the graph based semantic parsing work done by \cite{reddy2014large}. In this paper, exploiting information from the knowledge base in preliminary steps of the algorithm allows them to drastically reduce the search space, making the method efficient.
% As shown in Figure \ref{fig:yihFamilyGuy} rounded rectangles are the main topics, $y$ is the question which here is \textit{who}, $x$ is the possible answer and the diamond shape consist \textit{argmin} is a constraint that tells the model to return the first result. The authors believed that their CNN model using bag of letter-trigram has two advantages over the word embedding approach as described in \cite{bordes2014open}. Firstly, letter-trigrams capture sub-word semantics which helps the model to understand the possible errors in typing. It also controls the dimensionality of the input space due to the fixed size hashing. This makes it easier to scale to larger vocabulary. Second, it allows the use of deeper architectures employing convolution and max-pooling providing better representational power. In this paper, they formulate semantic parsing as making a query graph. It is done using search based techniques with states and actions in which the state is a possible parse and actions provide ways to grow the graph. The graph is grown by adding constraints which must be satisfied by the answer.  Neural networks are used to measure semantic similarity for the purpose of identifying core inferential chains.
% The early grounding of entities using the KB allows a more focused search and also makes it easier to resolve subsequent predicates. 

% \section{Embeddings, Neural Networks and End to End Training}
% \label{sec:embed}
% In contrast to all previous work that was based on mapping between lexicalized phrases and logical predicates, \cite{yang2014joint} proposed using an approach based on embeddings. Low-dimensional embedding of n-grams, entity type and predicates are learned jointly from knowledge base as well as from entries that are extracted from natural language texts that involve a subject, natural language relation and object. These entries correspond to triples in the KB of the form subject, predicate, object. The embeddings thus formed are used for judging the rank of the candidate logical forms that are generated. They are judged based on the similarity between the embeddings of the words in the natural language query and embeddings of the logical features that are in the generated structured logical queries. According to this ranking, the answers are finally retrieved from the knowledge base.  
%  They use a ranking loss \cite{weston2010large} where the score of positive pairs(observed pairs) in the training set should be more than that of the negative ones. Stochastic gradient descent is used to optimize the model's parameters.



% \cite{bordes2014question} and \cite{bordes2014open} . 




% Late last year, \cite{zhong2017seq2sql} released a large hand annotated data set of natural language to SQL pairs with the associated tables. This was an order of magnitude bigger than any existing data set for this task, spurring a lot of work in this area. In their associated paper, the authors proposed a sequence to sequence approach to solving this task where the input to the model consisted of words from the question, the columns of the table and the set of all SQL keywords. They rely on the assumption that the generated program will have words that are a subset of the words in this input word sequence. This is a strong assumption to make, as it is not always true that while asking questions, a user would use exactly the same words as the column names or that the words in the question will exactly map to entries in some row of the table. In order to train their model they use a combination of cross entropy loss for parts of the query with policy based reinforcement learning using in the loop query execution for the others. 
% In another effort to convert from natural language to SQL, \cite{sun2018semantic} propose to use three categories as their building blocks for the output parse corresponding to the structure of a SQL query as well as of the table. These three categories that they refer to as "channels" are used to fill in the column value, cell value and SQL keyword sections of a SQL query. The main contribution of this work beyond that of \cite{zhong2017seq2sql} is that by first selecting one of these three channels, the authors ensure that the predicted word is a complete entity that is either a cell in the table, a column in the table or a SQL keyword, instead of predicting each word separately.  


% Additions - not sure where to put it : 1. Sequential and conversational QA. 2. He He work on dialog systems


==> Semantic parsing survey/sections/task.tex <==
\label{sec:term}
Semantic parsers map \emph{natural language} (NL) utterances into a \textit{semantic representation}. These representations are often (interchangeably) referred to as logical forms, meaning representations (MR) or programs (\S~\ref{sub:logical_forms}). The representations are typically executed against \textit{an environment} (or context) (\S~\ref{sub:env}) (e.g. a relational knowledge base) to yield a desired output (e.g. answer to a question). The meaning representations are often based on an underlying formalism or \textit{grammar} (\S~\ref{sub:grammar}). The grammar is used to \emph{derive} valid logical forms. A \textit{model} is used to produce a distribution over these valid logical forms and a \textit{parser} searches for high scoring logical forms under this model. Finally, a \textit{learning algorithm} (\S~\ref{sec:learning}) is applied to update the parameters of the model, by using the training examples.
As a concrete example, consider the following from the WikiSQL dataset \cite{zhong2017seq2sql}. The goal of the semantic parser in figure~\ref{fig:overview} is to generate a valid \texttt{SQL} program (that can be derived from the grammar \cite{date1989guide}) given the natural language query and which produces the correct answer when executed against the table (context). Most published works also assume access to a deterministic executor (e.g. \texttt{SQL} interpreter) that can be called as many times as required. 
\begin{figure*}
    \centering
    \vspace{-2em}
    \includegraphics[width=0.85\columnwidth]{images/overview.pdf}
    \caption{Example of a semantic parsing task with various components.}
    \label{fig:overview}
\end{figure*}
\subsection{Language for Meaning Representation}
\label{sub:logical_forms}
The first main component of a semantic parsing framework is the language of the logical form or meaning representation. \\
\noindent \textbf{Logic based formalisms}: A straightforward language representation is one that uses \textit{first order logic} (FOL) --- consisting of quantified variables and functions that can only take objects as arguments. Following the examples from \citet{liang2016learning}, simple statements such as ``\textsc{all primes greater than 2 are odd}'' can easily be expressed in first order logic $\forall x .$\texttt{prime(x)}$\land$\texttt{more(x,2)}$\rightarrow$\texttt{odd(x)}. However FOL has limitations in its inability to represent and manipulate sets, for e.g. ``\textsc{Count the number of primes less than 10}'' cannot be expressed just with FOL. However, FOL augmented with \textit{lambda calculus} (LC) \cite{carpenter1997type} can be used to represent this --- \texttt{count}($\lambda$\texttt{x.prime(x)}$\land$\texttt{less(x,10)}), Here, $\lambda x$ denotes the \emph{set} of all x that satisfies a given condition. More details on the constituent units of lambda calculus can be found in \cite{artzi2013semantic}. LC has been used for querying databases \cite{zettlemoyer2005learning}, in implementing conversational agents \cite{artzi2011bootstrapping} as well as for providing instructions to robots \cite{artzi2013weakly}. \textit{Lambda Dependency based Compositional Semantics} ($\lambda$-DCS) by \citet{liang2013lambda}, is a more compact representation of LC. In this formalism, existential quantification is made implicit, allowing the elimination of variables. An example of this is ``\textsc{people above the age of 20}'' would be $\lambda x.\exists y.$ \texttt{AgeGreaterThan(x,y)}$\land$\texttt{Age(y, 20)} in LC and \texttt{AgeGreaterThan.Age.20} in $\lambda$-DCS. Readers are directed to \cite{liang2013lambda} for details. Several works such as \cite{berant2013semantic,pasupat2015compositional,krishnamurthy2017neural} use this formalism.\\
\noindent \textbf{Graph based formalisms}: Here the semantic form of a NL utterance is represented as a labeled graph where the nodes usually denote entities/events and edges denote semantic relations between the nodes. Graph representation offers a few advantages over other representations --- (a) They are easy for humans to read and comprehend, when compared to e.g. a \texttt{SQL} program. (b) They tend to abstract away from the syntactic structure and can even not be anchored to the words in the sentence. For example in Abstract Meaning Representation (AMR) \cite{banarescu2013abstract}, the word ``graduation'' can be mapped to the sense ``\texttt{graduate-01}'' in Propbank \cite{kingsbury2002treebank}. (c) There exists a rich literature on graph algorithms which can be leveraged for learning. Examples of graph based formalisms are AMR, Universal Conceptual Cognitive Annotation (UCCA) \cite{abend2013universal}, Semantic Dependency Parsing \cite{oepen2015semeval} etc. Recently, \citet{kollar2018alexa} introduced the Alexa Meaning Representation language that aims to capture the meaning of spoken language utterances.\\
\noindent \textbf{Programming languages}:
Of late, there have been efforts to convert a natural language query directly to high-level, general purpose programming languages (PL) such as Python, Java, SQL, Bash. Converting into general purpose PLs has its advantages over converting into structured logical forms since (a) PLs are widely used in the developer community, (b) the structured logical forms have relatively simple schema and syntax, limiting their scope and are generally developed for a particular problem, making them domain specific. In terms of application, being able to generate PLs directly from natural language queries would result in smarter programming environments for developers, and more importantly would allow non-experts to integrate non-trivial software components in their products. This motivation is also in spirit with the emerging research area of automated machine learning (AutoML) \cite{feurer2015efficient}.
% More recently there have been efforts to convert natural language directly to SQL (structured query language) which has long been an established formalism used by both industry and academia to query databases. An example of this is \textit{Number of medals that USA won in the 2008 Olympics} could be translated according to the schema as \texttt{SELECT COUNT Medals FROM Olympics WHERE Country = "USA" AND Year = "2008"}. 
% 
\subsection{Grammar}
\label{sub:grammar}
The grammar is a set of rules whose function is to define a set of candidate derivations for each natural language utterance. The type of grammar used decides the expressivity of the semantic parser as well as the computational complexity associated with building it. When dealing with complex but well structured queries (e.g. GeoQuery \cite{zelle1996learning}), strict grammars like \textit{Combinatory Categorial Grammar}\footnote{An accessible tutorial on parsing with CCGs can be found at \url{https://yoavartzi.com/tutorial/}} \cite{ccg} having many rules provide computational advantage by virtue of generating fewer possible derivations \cite{zettlemoyer2005learning,zettlemoyer2007online, artzi2011bootstrapping, kwiatkowski2013scaling}. On the other hand, when the language is noisy, \textit{floating rules} have the advantage of being able to capture ill formed sentences such as those produced when dealing with crowd sourced utterances \cite{wang2015building}, at the cost of producing many more candidate derivations \cite{berant2014semantic,pasupat2015compositional}. Recent work on general purpose code generation (such as SQL, Python etc) leverage the well-defined grammar associated with the programming language by attempting to directly generate the Abstract Syntax Trees associated with them (\S~\ref{sub:code_gen}).

\subsection{Underlying context}
\label{sub:env}
All mappings from natural language to semantic representations are with respect to the underlying context or environment on which they are based. An example of this context is a knowledge base (e.g. Freebase \cite{bollacker2008freebase}) which is essentially a store of complex structured and unstructured data.  The context can also be a small knowledge store --- tables from Wikipedia \cite{pasupat2015compositional}, spreadsheets \cite{gulwani2012spreadsheet}, images \cite{suhr2017corpus} etc. --- or designed for special purpose application such as flight-booking \cite{hemphill1990atis}, geography related queries \cite{zelle1996learning} and robot navigation \cite{macmahon2006walk,artzi2013weakly}.
%
